ZigZag: Universal Sampling-free Uncertainty Estimation Through Two-Step Inference

Whereas the ability of deep networks to produce useful predictions has been amply demonstrated, estimating the reliability of these predictions remains challenging. Sampling approaches such as MC-Dropout and Deep Ensembles have emerged as the most popular ones for this purpose. Unfortunately, they require many forward passes at inference time, which slows them down. Sampling-free approaches can be faster but suffer from other drawbacks, such as lower reliability of uncertainty estimates, difficulty of use, and limited applicability to different types of tasks and data. In this work, we introduce a sampling-free approach that is generic and easy to deploy, while producing reliable uncertainty estimates on par with state-of-the-art methods at a significantly lower computational cost. It is predicated on training the network to produce the same output with and without additional information about it. At inference time, when no prior information is given, we use the network's own prediction as the additional information. We then take the distance between the predictions with and without prior information as our uncertainty measure. We demonstrate our approach on several classification and regression tasks. We show that it delivers results on par with those of Ensembles but at a much lower computational cost.

==> bib/figmacro.tex <==
\newif\ifrgb
\rgbfalse

\newif\iffig
\figtrue

\newcommand{\figx}[2]
{
 \iffig
  \includegraphics[width=#1,keepaspectratio]{#2} 
 \else
   \parbox{#1}{#2} 
 \fi
}

\newcommand{\figy}[2]
{
 \iffig
  \includegraphics[height=#1,keepaspectratio]{#2}  
   \else
  \parbox{#1}{#2} 
 \fi
}

\newcommand{\figxy}[3]
{
 \iffig
  \includegraphics[width=#1,height=#2]{#3} 
 \else
   \parbox{#1}{#2}
  \fi
}

\newcommand{\figurecaption}[2]
{
\caption[]{\parbox[t]{#1}{#2}}
}

\newcommand{\fcaption}[1]
{
 \figurecaption{0.9\linewidth}{\small #1}
}

\newcommand{\figdir}[1]
{
\def\figurepath{#1}
}

\renewcommand{\topfraction}{1}
\renewcommand{\dbltopfraction}{1}
\renewcommand{\bottomfraction}{1}
\renewcommand{\textfraction}{.0}
\renewcommand{\floatpagefraction}{1}
\renewcommand{\dblfloatpagefraction}{1}


==> bib/report.tex <==
\usepackage{named}

\usepackage{geometry}
\usepackage{times}
\usepackage{graphics}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{amsthm,amssymb}
\usepackage{color}

\geometry{
 a4paper,
 left=21mm,
 right=21mm,
 top=16mm,
 bottom=16mm,
 }
 
%\setlength{\oddsidemargin}{0.0in}
%\setlength{\topmargin}{-0.125in}
%\setlength{\textwidth}{6.25in}
%\setlength{\textheight}{8.75in}
%\parskip 6pt plus 3pt minus 2pt

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\im}{\item}
\newcommand{\comment}[1]{}
\newcommand{\missing}[1]{\begin{large} {\bf ADD:} {\em #1} \end{large}}
\newcommand{\note}[1]{\begin{center} \noindent\framebox{\begin{minipage}{8cm}{\bf #1}\end{minipage}}\end{center}\\}
\newcommand{\rmk}[1]{{\color{red}{ \bf #1}}}
\newcommand{\red}[1]{{\color{red}{#1}}}
\newcommand{\url}[1]{#1}

\newif\ifsubmit
\submitfalse

\newif\ifdraft
\draftfalse

\newcommand{\dspace}{\renewcommand{\baselinestretch}{1.5}\large\normalsize}
\newcommand{\sspace}{\renewcommand{\baselinestretch}{1.0}\large\normalsize}
\newcommand{\Section}[1]{\section{#1}}
\newcommand{\SubSection}[1]{\subsection{#1}}
\sspace

\renewcommand{\floatpagefraction}{1.0}


==> fig/cars.tex <==
% !TEX root = ../top.tex
% !TEX spellcheck = en-US

% \begin{figure}[ht]
%     \vspace{-3mm}
%     \includegraphics[width=0.40\textwidth]{images/cars.png} \\
%     \includegraphics[width=0.35\textwidth]{images/unc_cars.png}
%     \centering
%     \vspace{-3mm}
%     \caption{\small {\bf Top: Pressure values.} The car dataset comprises many regular vehicles (left) and a few  streamlined ones  (right), which we treat as being out-of-distribution. Red and blue denote high and low pressures respectively.
%     {\bf Bottom: Pressure differences.} Large differences in predicted pressure are shown in red and low ones in blue. Ensembles (left) and ZigZag (right) yield the same pattern, with large values mostly  in high-curvature areas.}
%     \label{fig:cars}
% \end{figure}

\begin{figure}[ht!]
    \centering
    % \hspace*{-0.3cm}
    \begin{tabular}{@{}c@{}c@{}}
      \includegraphics[width=0.6\textwidth]{images/cars.png} &
      \includegraphics[width=0.4\textwidth]{images/unc_cars.png}
    \end{tabular}
    % \vspace{-4mm}
    \caption{\small {\bf Left: Pressure values.} The car dataset comprises many regular vehicles (left) and a few  streamlined ones  (right), which we treat as being out-of-distribution. Red and blue denote high and low pressures respectively.
    {\bf Right: Pressure differences.} Large differences in predicted pressure are shown in red and low ones in blue. Ensembles (left) and ZigZag (right) yield the same pattern, with large values mostly  in high-curvature areas.}
    \label{fig:sampling}
\end{figure}

==> fig/preg.tex <==
% \begin{figure}[ht]
%     \includegraphics[width=0.45\textwidth]{images/profiles.png}
%     \centering
%     \vspace{-3mm}
%     \caption{\small {\bf Airfoil Samples.} Training and testing profiles (\textbf{left}) have reasonable level of aerodynamics, whereas out-of-distribution samples (\textbf{right}) include only top-notch, but rare, shapes in terms of lift-to-drag ratio. The black arrows represent pressures while the red lines depict overall lift and drag. 
%     }
%     \label{fig: airfoils}
% \end{figure}

% \begin{figure}[ht]
%     \vspace{-3mm}
%     % \includegraphics[width=0.40\textwidth]{images/cars.png} \\
%     \includegraphics[width=0.35\textwidth]{images/unc_cars.png}
%     \centering
%     \vspace{-3mm}
%     \caption{\small {\bf Top: Pressure values.} The car dataset comprises many regular vehicles (left) and a few  streamlined ones  (right), which we treat as being out-of-distribution. Red and blue denote high and low pressures respectively.
%     {\bf Bottom: Pressure differences.} Large differences in predicted pressure are shown in red and low ones in blue. Ensembles (left) and ZigZag (right) yield the same pattern, with large values mostly  in high-curvature areas.}
%     \label{fig:cars}
% \end{figure}

\begin{figure}[ht]
    \centering
    \begin{subfigure}{.30\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/profiles.png}
        \caption{{\bf Airfoil Samples.} Training and testing profiles (left) have a reasonable level of aerodynamics, whereas out-of-distribution samples (right) include only top-notch, but rare, shapes in terms of lift-to-drag ratio. The black arrows represent pressures while the red lines depict overall lift and drag.}
        \label{fig:airfoils}
    \end{subfigure}%
    \hspace{5mm} % Adjust space between figures as needed
    \begin{subfigure}{.65\textwidth}
        \centering
        \includegraphics[width=\textwidth]{images/unc_cars.png}
        \caption{{\bf Top: Pressure values.} The car dataset comprises many regular vehicles (left) and a few streamlined ones (right), which we treat as being out-of-distribution. Red and blue denote high and low pressures respectively. {\bf Bottom: Pressure differences.} Large differences in predicted pressure are shown in red and low ones in blue. Ensembles (left) and ZigZag (right) yield the same pattern, with large values mostly in high-curvature areas.}
        \label{fig:cars}
    \end{subfigure}
    \caption{Combined caption for both figures.} % Optional: Overall caption for both subfigures
\end{figure}
